A small footprint travelling-wave parametric amplifier with a high Signal-to-Noise Ratio improvement in a wide band

We characterise a small footprint travelling-wave parametric amplifier (TWPA). The TWPA is built with magnetically flux-tunable superconducting nonlinear asymmetric inductive elements (SNAILs) and parallel-plate capacitors. It implements three-wave mixing (3WM) with resonant phase matching (RPM), a small cutoff frequency for high gain per unitcell and impedance matching networks for large bandwidth impedance matching. The device has 200 unitcells and a physical footprint of only 1.1 mm^2, yet demonstrates an average parametric gain of 19 dB over a 3 GHz bandwidth, an average effective signal-to-noise ratio improvement of 10 dB and a clear speedup of qubit readout time.

==> settings/usetikzext.tex <==

%%%%%%%% TO AVOID REDRAWING ALL TIKZ-FIGURES EVERY TIME! %%%%%%%%
\usetikzlibrary{external}
\tikzexternalize[prefix=tikzpics/tikzoutput/, optimize command away=\includepdf]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\simpletikz[1]{\tikzset{external/export next=false} 
\begin{tikzpicture}\input{tikzpics/#1}\end{tikzpicture}}
\newcommand\heavytikz[1]{\tikzset{external/export next=true} 
\begin{tikzpicture}\input{tikzpics/#1}\end{tikzpicture}}


==> tikzpics/DeviceFigure.tex <==
\onecolumngrid

\begin{figure}[H]
    \centering
    \simpletikz{Device.tikz}
    \caption{
        \textbf{The measured device.}
        The TWPA with its impedance matching networks
        on a silicon substrate with the dimensions 5\,mm\(\times\)10\,mm.
        The two impedance matching networks take up a total space of \(0.04\)\,mm\(^2\)
        and the TWPA itself, with its 200 unitcells, a space of 0.71\,mm\(^2\).
        When including a ground plane on each side with the total width of one RPM feature,
        the total physical size of the device is 1.1\,mm\(^2\).
    }
    \label{fig:Device}
\end{figure}

\twocolumngrid

==> tikzpics/NoiseModel.tex <==
\onecolumngrid

\begin{figure}[H]
    \centering
    \simpletikz{DetailedNoiseModel3.tikz}
    \caption{
        \textbf{Simple noise model.}
    }
    \label{fig:SimpleNoiseModel}
\end{figure}

\twocolumngrid
